M6: A Chinese Multimodal Pretrainer

In this work, we construct the largest dataset for multimodal pretraining in Chinese, which consists of over 1.9TB images and 292GB texts that cover a wide range of domains. We propose a cross-modal pretraining method called M6, referring to Multi-Modality to Multi-Modality Multitask Mega-transformer, for unified pretraining on the data of single modality and multiple modalities. We scale the model size up to 10 billion and 100 billion parameters, and build the largest pretrained model in Chinese. We apply the model to a series of downstream applications, and demonstrate its outstanding performance in comparison with strong baselines. Furthermore, we specifically design a downstream task of text-guided image generation, and show that the finetuned M6 can create high-quality images with high resolution and abundant details.

==> 3.task.tex <==
\section{Experiments}
\label{experiments}

In this section, we introduce our experiment settings and results on both multimodal and NLP downstream tasks. 
We also provide some analyses and case studies. 

\subsection{Downstream Tasks}
\begin{table}
  \caption{Results on the FMIQA dataset. We report both the overall accuracy and the accuracy on specific question types.} 
  \label{tab:fmiqa_result}
  \begin{tabular}{cccccc}
    \toprule
        Model   & Detection & Relation & Color & Number & Overall \\
        \midrule
        baseline    & 74.0  & 64.5  & 69.0  & 41.9  & 66.8  \\
        M6-base     & 79.0  & 71.0  & 70.9  & 45.2  & 71.0  \\
        M6-large    & \textbf{83.0}  & \textbf{77.4}  & \textbf{72.7}  & \textbf{48.4}  & \textbf{74.7}  \\
    \bottomrule
  \end{tabular}
\end{table}

\subsubsection{Multimodal Downstream Tasks} 
We compare M6 with competitive baselines on several multimodal downstream tasks, including visual QA, image-text matching and image captioning. These tasks evaluate the model's ability on cross-modal understanding from various perspectives.


\vpara{Visual Question Answering}
% One evaluation of the model's capability of cross-modal understanding stands on the tasks related question answering with visual information. 
We leverage the FMIQA dataset \cite{fmiqa} as the Chinese visual QA benchmark, which requires the model to generate the answer given an image and a question. 
% Since FMIQA can still be viewed as a generation task given the visual context, there is no need to add extra modules to M6. 
% Conditioned on the input image, the question concatenated with the answer text is taken as the generation target during finetuning. 
% The language modeling objective is used. 
% In evaluation, the question is input as the prompt with the image. 
We implement a transformer-based model as our baseline. 
For the evaluation, we split the test set manually by random sampling 200 from the dataset as there is no official release of the test set, and we evaluate the overall accuracy by human evaluation. 
% The answer generated by the model is manually evaluated as correct or wrong based on the ground truth answer. The overall accuracy on the test set is used as the evaluation metric.
% For visual QA, 
% We ask several annotators to determine whether the model output is correct. 
The results are demonstrated in Table~\ref{tab:fmiqa_result}. 
The pretrained M6-base outperforms the baseline by a large margin (+6.2\%), which indicates the effectiveness of multimodal pretraining. 
Scaling up the model to M6-large further brings 5.2\% improvement. 

To carefully inspect the benefit of pretraining, we also report the accuracy scores on different types of questions. 
We find that M6-base greatly improves the baseline by 10.1\% on the questions about the spatial relations between the objects. 
Meanwhile, M6-base surpasses the baseline by 7.9\% on the counting questions, indicating that the pretraining may facilitate numeric reasoning. The pretraining achieves 6.8\% improvement on the questions related to the object and action detection. 
Interestingly, we find the improvement on color recognition questions is relatively marginal (+2.8\%), which may reflect that pretraining contributes little to the ability of color recognition. 

\vpara{Image-text Matching}
\begin{table}
  \caption{Results on the E-Commerce ITM dataset. We report the accuracy on the test set.} 
  \label{tab:itm_result}
  \begin{tabular}{ccc}
    \toprule
        Model   & Accuracy & Delta \\
        \midrule
        InterBert & 81.8  & - \\
        M6-base     & \textbf{90.2}  & 8.4 \\
    \bottomrule
  \end{tabular}
\end{table}
% Another important evaluation is on the model's ability in cross-modal matching. 
We evaluate the model's ability in cross-modal retrieval. 
Specifically, we construct a dataset (named E-Commerce ITM) containing pairs of texts and images from the mobile Taobao. 
Each pair belongs to a single item. 
More details of the data statistics and data processing are referred to the appendix. 
% The query and product image in a pair can be relevant or irrelevant, which requires the model to classify. 
We require the model to perform binary classification to discriminate positive and negative samples. 
% For this task, we add an extra-layer for binary classification on top of the M6 backbone. 
% Given the query-image pair, the generated representation at the ending position is sent into the layer as it is able to receive information from the whole context with attention mechanism. The model  is finetuned with cross-entropy. 
We compare our model with InterBert~\cite{interbert}, which is also a Chinese multi-modal pretrained model effective in cross-modal classification downstream tasks. The InterBert utilizes object-based features and has been pretrained on Taobao product image-text data as well.
% We compare our model with FashionBert, which is a single-stream multi-modal pretrained model and specifically designed for cross-modal retrieval \cite{fashionbert}.
%And as mentioned above, it takes patch features as visual inputs. 

\begin{table}
  \caption{Results on the E-Commerce IC dataset.} 
  \label{tab:ic_result}
  \begin{tabular}{cccc}
    \toprule
        Model   & Grammar & Correctness & Coherence \\
        \midrule
        baseline    & 4.3  & 2.1  & 3.0 \\
        M6-base    & \textbf{4.5}  & \textbf{3.0}  & \textbf{3.6} \\
    \bottomrule
  \end{tabular}
\end{table}

The results are shown in Table~\ref{tab:itm_result}. 
It should be noted that the InterBert and M6-base are both implemented with transformer-based architecture and have similar model scale. 
However, M6-base still outperforms InterBert by 9.3\%.
In experiments, we find the product images generally contain relatively fewer detected objects, which may harm the performance on this task. 
In contrast, M6 avoids this problem by employing the patch features and achieves much better performance.
% This indicates the superiority on cross-modal understanding which multi-task pretraining and larger pretraining corpus may bring.

\vpara{Image Captioning} 
% The most typical task of cross-modal generation is image captioning.
Image captioning requires the model to generate a caption that describes the given image, which examines the model ability of cross-modal generation. 
We construct a dataset (named E-Commerce IC) containing pairs of product descriptions and product images from Taobao. 
More details of the construction of the finetuning dataset are referred to the appendix. 
We finetune the model with the image-to-text transfer task. 
At the stage of inference, we apply beam search with a beam size of 5. 
% The beam search width during decoding is set to 5.
We compare our model with a baseline of transformer in the human evaluation. 
We ask several annotators with linguistic background to evaluate from three perspectives: grammar (whether a text is fluent without grammatical error), correctness (whether a text is faithful to the image), coherence (whether a text is logically coherent and well-organized). During the evaluation, we randomly sample 100 images from the test set. For each image, an annotator is asked to score the text generated by different models. The scores are within the range of $[0,5]$. 

The results on Table \ref{tab:ic_result} show that M6-base outperforms the baseline in all of the metrics. 
We find that all models achieve high scores in grammar. However, in both correctness and coherence, M6-base outperforms the baseline model by a large margin (+42.8\% and +20.0\%), indicating that multimodal pretraining helps to generate more faithful and coherent texts. 

\begin{table}
  \caption{Zero-shot templates for NLP downstream tasks. Words in bold denote the input text.  }
  \label{tab:zeroshot_templates}
  \centering
  \begin{tabular}{cc}
    \toprule
        Datasets & Templates\\
        \midrule
        \multirow{2}{*}{TNEWS} &  标题:\textbf{title};关键词:\textbf{keywords};分类:\textbf{label} \\
          & Title:\textbf{title};Keywords:\textbf{keywords};Label:\textbf{label}   \\
         \multirow{2}{*}{ChID} & 成语填空:... \textbf{prefix} [MASK] \textbf{postfix}...\\
        & Idiom cloze:... \textbf{prefix} [MASK] \textbf{postfix}...  \\
        \multirow{2}{*}{CMRC2018} & \textbf{paragraph} 问题: \textbf{question}? 回答:  \\ 
        & \textbf{paragraph} Question: \textbf{question}? Answer: \\
      %  OCNLI & 句子``\textbf{premise}''与句子``\textbf{hypothesis}''的关系是\textbf{label} & The relationship between ``\textbf{premise}'' and ``\textbf{hypothesis}'' is \textbf{label} \\
        % RefCOCO+ & i:20K, t:141K & - & - \\
        % KDD Cup & i:3M, t:3M & i:15K, t:0.5K & i:30K, t:1K \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}
  \caption{Results of the models on the three NLP downstream tasks with zero-shot settings. The results of the baselines are those reported in their original papers. \textit{Random} denotes randomly choosing from the candidate lists.}
  \label{tab:zero-shot results}
  \begin{tabular}{ccccc}
    \toprule
    
        \multirow{2}{*}{Models} &\multirow{2}{*}{$n_{param}$} & TNEWS   & {CMRC}  & CHID \\
                  &      & Acc.  & F1  & Acc. \\
        \midrule
        Random     & -        & 25.0  & -   & 10.0 \\
%        CPM-small  & 109M & 62.6   & 6.03& 0.20 &43.3\\
        CPM-medium & 334M & 61.8  &8.60 &52.4\\
        CPM-large  & 2.6B & 70.3 & 13.37 &\textbf{68.5}\\
        M6-base   & 327M & 65.5 & 13.58 & 61.7\\
        M6-large  &  10B & \textbf{72.7}  & \textbf{13.88}   & 65.3 \\
    \bottomrule
  \end{tabular}
\end{table}

\subsubsection{NLP Downstream Tasks}
We focus on the evaluation of the zero-shot learning of our model on several NLP downstream tasks, including text classification, reading comprehension, and cloze.
M6 is compared with the recent largest published Chinese Pretrained Language Model~\citep{zhang2020cpm}, which consists of around 2.6B parameters and has achieved strong performance on many NLP downstream tasks in the settings of zero-shot.
The templates we used for zero-shot settings are shown in Table \ref{tab:zeroshot_templates}.
Results on these NLP downstream tasks are shown in Table \ref{tab:zero-shot results}.

\vpara{Text Classification}
We first evaluate the model's zero-shot ability on text classification tasks.
This task requires the model to categorize text~(e.g. sentences, paragraphs, or sentence pairs) into organized groups. 
We conduct our experiments on TouTiao News Titles Classification (TNEWS)~\citep{xu2020clue}.
We calculate the perplexity of each candidate sentence-label pair of the validation dataset.
Pairs with the lowest perplexities are treated as the predictions.
Following \citet{zhang2020cpm}, we convert the original tasks to the task of 4-way classification tasks with 3 negative samples for better efficiency as there are more than 10 kinds of labels.
We repeat this procedure three times to make the result more stable and report the average accuracy.

Experimental results show that M6-base outperforms CPM-medium by 4.6\% on TNEWS.
M6-large further surpasses CPM-large by 3.3\% and achieves a new state-of-the-art, even if it is pretrained with much fewer samples.
This indicates that our models have better understanding of the semantic differences of labels in different categories. 

\vpara{Reading Comprehension}
A span-extraction dataset for Chinese Machine Reading Comprehension (CMRC2018) is chosen to evaluate the model's ability of single-modal understanding \cite{cui2018span}.
This task requires the model to extract spans from the given passages to answer several questions.
We concatenate the given passage and one of the following questions as the input of M6 pretrained models.
Slightly different from the original extracting task, we ask the model to generate an answer according to the input text freely.

Our M6 models show comparable performance with CPM-large on Reading Comprehension.
However, without finetuning, M6 models are more likely to generate a long sentence to answer the given question which may limit the improvement in F1-score when scaling up the model to M6-large.



\vpara{Cloze}
This task requires the model to choose the correct word from the given candidate lists to fill in the blanks. 
We conduct experiments on the Chinese IDiom cloze test dataset (ChID)\cite{zheng2019chid}. 
In this task, we utilize a pattern similar to the pretraining task of text denoising.
The blank in the passage is replaced by the token ``[MASK]'' in the encoder input and is replaced by each idiom from the given candidate list in the decoder input.
A similar procedure as mentioned above is applied to get predictions.

With the help of text denoising, M6-base outperforms CPM-medium by a large margin (17.7\%).
Our model can have a better view of the whole passage with the bi-directional attention compared with CPM which only uses single-directional attention.
However, limited by hardware conditions, passages longer than 256 tokens are truncated when we evaluate our models on CHID.
This makes the performance of the M6-large not further improved compared with that of the M6-base. 
Another possibility is that the insufficient pretraining affects the performance of the large model. 
We have found that the more samples that it has been pretrained, the higher performance it can achieve. We demonstrate the relevant details in the appendix. 

==> 4.4.long-text.tex <==
\subsection{Product Description Generation}

\subsubsection{Additional Examples}

% \begin{figure}[tb]
%     \centering
%     \includegraphics[width=0.47\textwidth]{pic/M6_case_v2_2.pdf}
%     \caption{ Another example of general visual question answering. }
%     \label{fig:i2t_case2}
% \end{figure}

\begin{figure}[tb]
    \centering
    \includegraphics[width=0.47\textwidth]{pic/i2t.pdf}
    \caption{Two examples of image caption. We only use the image feature as input and provide no prompt. } 
    \label{fig:i2t_case3}
\end{figure}


\begin{figure}[tb]
    \centering
    \includegraphics[width=0.47\textwidth]{pic/txt_cnt.pdf}
    \caption{One example of continue writing. We simply take the context as prompt. }
    \label{fig:t2t_case}
\end{figure}


Our pretrained model has strong capability of performing different tasks by providing different prompts.
We further show how the model performing other generation tasks including image caption and continue writing in Figure \ref{fig:i2t_case3} and Figure \ref{fig:t2t_case}.
